Conductance-based dendrites perform Bayes-optimal cue integration

A fundamental function of cortical circuits is the integration of information from different sources to form a reliable basis for behavior. While animals behave as if they optimally integrate information according to Bayesian probability theory, the implementation of the required computations in the biological substrate remains unclear. We propose a novel, Bayesian view on the dynamics of conductance-based neurons and synapses which suggests that they are naturally equipped to optimally perform information integration. In our approach apical dendrites represent prior expectations over somatic potentials, while basal dendrites represent likelihoods of somatic potentials. These are parametrized by local quantities, the effective reversal potentials and membrane conductances. We formally demonstrate that under these assumptions the somatic compartment naturally computes the corresponding posterior. We derive a gradient-based plasticity rule, allowing neurons to learn desired target distributions and weight synaptic inputs by their relative reliabilities. Our theory explains various experimental findings on the system and single-cell level related to multi-sensory integration, which we illustrate with simulations. Furthermore, we make experimentally testable predictions on Bayesian dendritic integration and synaptic plasticity.

==> supplements_supplements_raw.tex <==
\hrule
\vspace{0.5cm}
{\bf \Huge Drop?}
\vspace{0.5cm}
\hrule

\section{Somatic update reflects Bayesian inference}
%=======================

The intrinsically biderectional somato-dendritic voltage diffusion can be mapped to the Bayesian inversion of a generative distribution as illustrated in Fig.\ref{fig:SI_Fig1}.

In the main text we describe the somatic voltage dynamics (Eqn.~\ref{eq:Cus}) as a stochastic voltage sampling scenario with fixed dendritic input. By virtue of the Gaussian noise $\xi \,$ defined in Eqn.~\ref{eq:results-dynamics-soma}, the somatic voltage $u_s$ stochastically samples around the mean $\bar E_s$ with variance $\lambda_s / \bar g_s$. In this scenario, the fixed presynaptic rates $r$ encode a presynaptic stimulus, and through the dendritic conductances $g^\E_d(r)$ the soma pools the dendritic opinion about how likely the neuronal feature is present in $r$. There is a single prior $p( u_s | \Eprior, \gprior )$ before sampling the dendritic input, a single presynaptic stimulus $r$ generating the pairs $(E_d, g_d)$ for the dendrites $d=1,...,D$, and there is a single posterior $p(\us \,|\, \Eprior, \gprior, E_{\bf d}, g_{\bf d})$.  

There is an alternative scenario that considers stochastic dendritic opinions centered around $E_d$, but endowed with dendrite-specific noise.  In this scenario, the noise $\xi$ in Eqn.~\ref{eq:results-dynamics-soma} is produced by independent dendritic Gaussian noises $\xi_d$, each of variance $2C \lambda_\text{e}\alpha_{sd} \, g_d / \bar g_s$ with $\bargs = \sum_{d=0}^D \alphasd g_{d}$. The noise also includes a somatic contribution $\xi_s$. Hence, we can write $\xi = \sum_{d=0}^D \, \xi_d$. The variance of $\xi$ is the sum of the individual variances, $\mathrm{var}(\xi) = \sum_{d=0}^D \mathrm{var}(\xi_d) = 2C \lambda_\text{e}$. In the stochastic steady state (Eqn.~\ref{eq:ps1}), the somatic voltage fluctuates around $\langle u_s \rangle = \barEs =  \frac{1}{\bargs} \sum_{d=0}^D \alphasd g_{d} E_{d} $ with variance $\sigma_\text{s}^2  =  \lambda_\text{e} / \bargs $. In this dendritic noise scenario, the somatic prior is continuously updated by the new dendritic opinions. It turns into a posterior that is also a prior for the next update.

\section{``On variance''}

\todoin{JJ: moved from methods}
The error in the dendritic estimate $\frac{\lambda_\text{e}}{\bargs}$ of the somatic variance sampled by $(\us^* - \barEs)^2$ vanishes in average when discarding the somatic nudging, $\frac{\lambda_\text{e}}{\bargs} - \langle (\us - \barEs)^2 \rangle = 0$ for $\beta=0$. This is because in the voltage dynamics $\tau \, \dotus =  \barEs - \us + \frac{1}{\bargs}\xi$ with $\tau = C/\bargs$, see Eqn.~\ref{eq:results-dynamics-soma}, the variance $\sigma_I^2 = 2 C\,\lambda_\text{e} /\bargs^2$ in the Gaussian input $\xi/\bargs$ translates into a variance $\sigma_\text{s}^2 = \sigma_I^2 / (2 \tau) = \lambda_\text{e} / \bargs $ of $\us$ \cite{vankampen1992stochastic}. Hence, the total conductance dynamically estimates the voltage variability.
